Decision-Point Guided Safe Policy Improvement

Within batch reinforcement learning, safe policy improvement (SPI) seeks to ensure that the learnt policy performs at least as well as the behavior policy that generated the dataset. The core challenge in SPI is seeking improvements while balancing risk when many state-action pairs may be infrequently visited. In this work, we introduce Decision Points RL (DPRL), an algorithm that restricts the set of state-action pairs (or regions for continuous states) considered for improvement. DPRL ensures high-confidence improvement in densely visited states (i.e. decision points) while still utilizing data from sparsely visited states. By appropriately limiting where and how we may deviate from the behavior policy, we achieve tighter bounds than prior work; specifically, our data-dependent bounds do not scale with the size of the state and action spaces. In addition to the analysis, we demonstrate that DPRL is both safe and performant on synthetic and real datasets.

==> algorithms/dp_continuous.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
    \begin{minipage}{0.5\textwidth}
      \begin{algorithm}[H]
        \caption{DPRL-C for Continuous States}
        \label{alg:dp_continuous}
        \begin{algorithmic}[1]
        \STATE \textbf{Input:} State $s$
        \STATE \textbf{Input:} BallTree$_s$($\cdot, \gD, r$), BallTree$_s$($\cdot, \gD, r$)
        \STATE $\gN(s) \leftarrow$ BallTree$_s$($s, \gD, r$)
        \STATE $\gN(s,a) \leftarrow$ BallTree$_{sa}$($(s,a), \gD, r$) for all $a \in \gA$
        \IF{$\abs{\gN(s)} \leq \Nmin$}
            \STATE \textbf{Output:} DEFER
        \ELSE
            \STATE Compute $\hat{V}^{\pi_b}(s)$ using $\gN(s)$
            \STATE Compute $\hat{Q}^{\pi_b}(s, a)$ using $\gN(s, a)$
            \STATE Compute $\gAdp_s$ using Eq~\ref{eq:advantageous_actions_continuous}
            \IF{$\gAdp_s = \emptyset$}
                \STATE \textbf{Output:} DEFER
            \ELSE
                \STATE \textbf{Output:} $\argmax_{a \in \gAdp_s} \hat{Q}^{\pi_b}(s, a)$
            \ENDIF
        \ENDIF
        \end{algorithmic}
    \end{algorithm}
    \end{minipage}
\end{wrapfigure}

==> algorithms/dp_discrete.tex <==

    
        

==> src/related_work.tex <==


% \subsection{Notes on baselines}
% \begin{enumerate}
%     \item SPIBB \citep{larocheSafePolicyImprovement2019} also uses the $\Nmin$ parameter to build a set of $(s,a)$-pairs which were observed less than $\Nmin$ times. However, it still puts probability (equal to $\pib(a|s)$) on $(s,a)$ pairs which were observed less than $\Nmin$ times. In contrast, DP is explicit in its improvements: it suggests action $a$ in state $s$ only (a) if it was observed at least $\Nmin$ times, and (b) if it leads to a better return than following $\pib(s)$. If it fails to find such an action, it defers to $\pib$. Furthermore, our policy-improvement bounds more tightly predict when the learned policies revert to $\pib$ (i.e. there is no improvement possible).
%     \item PQI \citep{liuProvablyGoodBatch2020c} uses the empirical state-action density $\hat{\mu}(s,a)$ to filter the $(s,a)$ pairs which are not frequent in the batch dataset. This is equivalent to DP in the discrete state case. In the continuous case experiments, they rely on heuristics to implicitly filter $(s,a)$ pairs that are infrequent. In contrast, we directly control the filtering using the $\Nmin$ and $r$ parameters. Another difference is that PQI builds a parametric estimate of $Q$ function, whereas DP builds a nonparametric estimate of the $Q$ function.
% \end{enumerate}

% Offline RL (high-confidence policy improvement)
% Count-based regularization methods 
% (Other) policy regularization methods
% (Other) value regularization methods

% ## Theory
% Discrete
% 	Model-based
% 	- SPIBB (Laroche et al Thm 2; soft-support w/ count-threshold) + follow-up work
% 	Model-free
% 	- PQI (Liu et al Cor 2; support-matching w/ density threshold)

% Continuous
% 	Model-based
% 	- Count-MOReL (Kim and Oh Thm 2 for pi_b; reward-penalization w/ counts)
% 	Model-free
% 	- PQI (Liu et al Thm 1; support-matching w/ density threshold)


% ## Baselines
% Count-based
% - SPIBB for discrete case (model-based, model-free; hparam: threshold for n(s,a))

% - 
% Conservative by making R pessimistic
% - Count-MOReL (Kim+Oh; Count-based conservatism) for discrete+continuous (model-based; hparam: penalty multiplier for reward (beta))
% - MOReL (model-based: hparam: threshold for T-uncertainty)

% Support-based
% - BCQL (model-free; Q-learning where argmax_a Q(s',a) is always within batch => pi constrained to support if Q is pessimistically initialized)

% Density-based
% - PQI (Liu et al) (model-free; hparam: threshold for d(s,a))
% - CQL (kumar et al 2020) (model-free; hparam: reg. penalty for matching Q-value under pi and pi_b)

% "Conservative" by constraining T close to T_MLE
% - RAMBO (model-based ; )

% No conservatism baseline
% - FQI

% No improvement baseline
% - BC

==> src/theory/asm_value_error.tex <==
\begin{assumption}[Value Error]
    \label{asm:value_error}
    For any $(s,a) \in \gS \times \gA$ and $\pi$, the value functions in the neighborhood of $(s,a)$ are bounded:
    \begin{gather}
        \sup_{s \in \gS, s' \in \gS}\frac{\abs{Q^\pi(s,a) - Q^\pi(s',a)}}{d(s,s')} \leq L_Q \\
        \sup_{s \in \gS, s' \in \gS}\frac{\abs{V^\pi(s) - V^\pi(s')}}{d(s,s')} \leq L_V
    \end{gather}
    TODO: Define $d(s,s')$, show how $L_Q$ and $L_V$ are related.
\end{assumption}
